An efficient structural attack on NIST submission DAGS

We present an efficient key recovery attack on code based encryption schemes using some quasi-dyadic alternant codes with extension degree 2. This attack permits to break the proposal DAGS recently submitted to NIST.

==> Conclusion.tex <==
\section*{Conclusion}
We provide a polynomial time attack on DAGS proposal. This attack
permits actually to recover the structure of any alternant
code with extension degree 2 and a permutation group such that
$\frac{q}{|\group|}$ is small.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Article"
%%% End:


==> Extensions.tex <==
\section{Extensions and reach of the attack}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Article"
%%% End:

